SPIDR: SDF-based Neural Point Fields for Illumination and Deformation

Neural radiance fields (NeRFs) have recently emerged as a promising approach for 3D reconstruction and novel view synthesis. However, NeRF-based methods encode shape, reflectance, and illumination implicitly and this makes it challenging for users to manipulate these properties in the rendered images explicitly. Existing approaches only enable limited editing of the scene and deformation of the geometry. Furthermore, no existing work enables accurate scene illumination after object deformation. In this work, we introduce SPIDR, a new hybrid neural SDF representation. SPIDR combines point cloud and neural implicit representations to enable the reconstruction of higher quality object surfaces for geometry deformation and lighting estimation. meshes and surfaces for object deformation and lighting estimation. To more accurately capture environment illumination for scene relighting, we propose a novel neural implicit model to learn environment light. To enable more accurate illumination updates after deformation, we use the shadow mapping technique to approximate the light visibility updates caused by geometry editing. We demonstrate the effectiveness of SPIDR in enabling high quality geometry editing with more accurate updates to the illumination of the scene.

==> introduction_v0.tex <==
\section{Introduction}
\begin{comment}
{\color{blue}
\begin{itemize}
    \item Motivate NeRF (small para)
    \begin{itemize}
        \item Deformation: motivate why it's important
    \end{itemize}
    \item What does NeRF not do well that you are trying to do:
    \item Deformation is challenging because:
    \begin{itemize}
        \item Lighting
        \item Manipulating the implicit representation is difficult
    \end{itemize}
    \item What has prior work done and not done (1 para)
    \item Our goal is to enable ... 
    \item What you did:
    \begin{itemize}
        \item SDF-based point Nerf for better surface
        \begin{itemize}
            \item Why is this beneficial
            \item Why is this is not so easy to implement
            \item How you solved it
        \end{itemize}
        \item Environment light ...
        \begin{itemize}
            \item Why is this beneficial
            \item Why is this is not so easy to implement
            \item How you solved it
        \end{itemize}
    \end{itemize}
    \item Anything else about the mechanism (deformations..) 
    \begin{itemize}
        \item Is it similar to other works? If so (cite)
        \item What is different?
        \item What is the benefit?
    \end{itemize}
    \item Results: Summary of the key results (also compared to prior work)
    \item Conclusions: Summarize any important contributions
\end{itemize}

}
\end{comment}
% Motivate NeRF (small para)
\noindent
%Scene modeling from image data and novel view rendering have been extensively studied in computer vision and graphics. 
Recent advancements in implicit neural representations of 3D scenes, such as signed distance fields (SDF) \citep{Park_2019_CVPR} and neural radiance fields (NeRF) \citep{mildenhall2020nerf}, have demonstrated exciting new capabilities in scene reconstruction and novel view synthesis. 
% Due to its high rendering quality, methods like NeRF now become a promising representation for 3D scenes and objects. 
Recent research has investigated various aspects of implicit representations including training/inference acceleration, generative synthesis, modeling dynamic scenes, and relighting \citep{dellaert2020neural}.
% Though promising, NeRF methods also have their limitations, preventing such representations from being integrated into the traditional graphics pipeline. % for artistic creations such as creating 3D content in games and movies. 
A key aspect of 3D representations is in their ability to be easily edited for tasks such as .... \ruofan{TODO}.
However, with implicit representations, the object geometry, texture, and environment light are all entangled in the learned parameters of the representation. Thus, the geometry and illumination of objects/scenes represented by NeRFs are fundamentally challenging to edit.  
For example, \ruofan{TODO} NeRFs cannot be edited by using .... as in traditional rendering pipelines with tools such Blender (cite). 
%Users cannot easily manipulate NeRF's rendered results like what they do in the traditional rendering pipeline (e.g., Blender). 
There are works trying to improve the shape editability of NeRF \citep{liu2021editing, Yuan22NeRFEditing, neumesh}. However, they cannot render correct environment illumination after object deformation.
On the other hand, works that estimate NeRF's environmental lighting \citep{nerv2021, nerfactor} do not support geometry editing.
% There are works focusing on different aspects of NeRF's editability, for example, editing shape and color with scribble \citep{liu2021editing}, material and illunimation editing \citep{nerv2021, nerfactor}, scene composition \citep{yang2021objectnerf, lazova2022control}, etc.
% However, most of them either perform badly when combined with other types of editing not mentioned in the paper (e.g., relighting works generally do not well support the shape editing)
% , or are still limited to rendering simple scenes \citep{liu2021editing} or relatively low rendering quality \citep{nerfactor}.
Therefore, further study on the editable and controllable NeRF representation is still required for NeRF's wide applications. % in artistic creation.

% What does NeRF not do well that you are trying to do:
There are two aspects of limitations we will consider in this paper. 
Firstly, NeRF-based methods use a neural function with spatial coordinates as the input to predict the corresponding geometry and radiance information. 
Since the implicitly represented scene or object relies on the decoded information from every sampled spatial coordinate in the object's modeling space, we cannot explicitly manipulate the geometry of the NeRF representation.
There are quite a few recent NeRF methods that adopt hybrid neural representations with the assistance of discrete representations (e.g., voxel grids, and hash tables). The use of explicit representations such as voxel grids can improve geometry editability, but it is still limited to the coarse-grained geometry deformation or composition.
%
Secondly, NeRF methods encode all the rendering parameters implicitly in their neural models, we do not have direct control of NeRF's illumination. Therefore, the deformation of object geometry in NeRF does not guarantee the change of illumination effects, e.g., unshadowed regions should become shadowed if light occlusion happens after the deformation, but the existing methods are unable to achieve such intuitive illumination change. 
% In the traditional graphics pipeline, the surface radiance is described by the rendering equation \citep{kajiya1986rendering} and is controlled by rendering parameters, e.g., the material's bidirectional reflectance distribution function (BRDF), environment light, surface visibility, etc.
%and the object geometry itself.
To make NeRF models aware of the change in lighting, those rendering parameters have to be decomposed or explicitly parameterized in NeRF's neural model.
However, this is a very challenging task, as discussed in other related works \citep{nerfactor, boss2021neural}, it not only requires high-quality object geometry for computing the surface normal and visibility but also learns a bunch of rendering parameters from a single unknown environment.

% What has prior work done and not done (1 para)
% Some recent works have tackled the general non-rigid geometry manipulation problem by combining implicit neural fields with explicit representations. 
Some recent works have tackled the NeRF's geometry deformation problem. 
% D-NeRF \citep{pumarola2021d} first proposes a way to learn dynamic scenes by warping the input coordinate space for implicit fields. Instead of changing the geometry of the learned object, this method "bends" the camera rays through the canonical implicit field representing a static object during volume rendering so that the deformed object is rendered. D-NeRF is a method for learning dynamic scenes from sequential images representing known deformations, and it does not support user-defined geometry manipulation. 
NeRF-Editing \citep{Yuan22NeRFEditing} provides flexible object deformation for NeRF.
this method extracts the mesh from a trained NeRF model from the static scene. Users can perform any deformation on the extracted mesh, then deformed the mesh guides the implicit field warping to achieve volume rendering of the deformed object. 
NeuMesh \citep{neumesh} is another concurrent work that learns a hybrid neural representation assisted with the mesh.
Since NeuMesh's neural features are bound to mesh vertices and interpolation on the local relative positions is used for sampled points, deformations made on their mesh can directly change the corresponding neural representation as well as the final rendered images. 
However, neither NeRF-Editing nor NeuMesh addresses the illumination updates after the deformation. Besides, both two methods rely on the trained pure implicit NeRF model (i.e., NeuS \citep{wang2021neus}) for the mesh extraction, which is relatively time-consuming and may not be able to capture high-frequency details for the sake of continuous SDF parameterization.
% 
There are also some recent works focusing on modeling NeRF's lighting and reflectance. These works either use the more complicated models to implicitly represent the reflectance \citep{yariv2020multiview, verbin2021ref} or decompose NeRF for learning a set of rendering parameters explicitly \citep{nerv2021, nerfactor, boss2021neural}. However, the main application of these works is scene relighting or material editing and none of them can be directly applied to object deformations. Even if NeRF deformation methods are used, these NeRF lighting methods still suffer from either relatively low rendering quality or incorrect surface lighting (e.g., changes of hard shadows).

%The user performs shape deformations on the mesh. For each sample point along the ray, they use the correspondence between the deformed mesh and original mesh to compute the sample point in the canonical space and estimate the rendered color. However, the NeRF model implicitly encodes all reflectance into its implicit volume, such methods creates obvious artifacts as indirect illumination and shadows were incorrectly updated. NeuMesh \citep{neumesh} encodes neural implicit field as latent code on mesh vertices, \haoda{TODO: method and limitations}. 

% Our goal is to enable ... 
% What you did:
Given these challenges, our \textbf{goal} is to achieve fine-grained geometry deformation and adaptive illumination updates for NeRF-based representations.
% enumeration.
To achieve this goal, we present an SDF-based hybrid NeRF model with additionally learned rendering parameters to facilitate lighting-aware object geometry editing. 
We further discussed our model from the following two aspects:  
\textbf{1)} For the representation part, our hybrid NeRF model is a combination of neural implicit representation and point cloud representation \citep{xu2022point}.
Because of such implicit-explicit hybrid representation, our model is able to update its represented geometry like NeuMesh, by directly manipulating the point cloud or the mesh registered with the point cloud. Since lighting and reflectance heavily rely on the high-quality reconstructed geometry, simply using a hybrid NeRF like Point-NeRF \citep{xu2022point} is still not enough.
In order to obtain better object surfaces and normals for the later BRDF-based rendering.
Our model adopts the signed distance function (SDF) based NeRF parameterization \citep{yariv2021volume, wang2021neus}. Using hybrid representation at the very beginning also makes our model less time-consuming compared to NeRF-Editing and NeuMesh, which requires the training of fully implicit NeRF models.
\textbf{2)} For the illumination part, we additionally learn BRDF parameters and environment light, based on the geometry and radiance learned from our hybrid NeRF model.
% More specifically, we use extra MLP branches to learn parameters for the microfacet BRDF model and another independent implicit coordinate-based MLP to represent HDR light probe image for the environment light.
%, Unlike other existing works \, cite{nerv2021, nerfactor} that use MLP to learn surface visibility, we directly use the visibility map that is efficiently computed by the shadow mapping technique.
%
However, unlike other existing works \citep{nerv2021, zhang2021physg, nerfactor}, we use another implicit coordinate-based MLP to represent HDR light probe image for better continuity; instead of learning high-dimensional visibility maps with MLP that is unable to update the object occlusion after deformation, we directly use the visibility map that is efficiently computed by the shadow mapping technique.


% and light decoupling from BRDF rendering to minimize reflectance artifacts. During volume rendering, we decode diffusion color, surface normal, and light visibility at each query point from neighboring points' neural features. \haoda{the rendering process needs update, need help from Ruofan?} Combining with the environmental light map, we perform a BRDF-based rendering process to obtain the final color. With the explicit point cloud representation, the user will be able to easily edit the shape either by directly manipulating point coordinates or by deforming the extracted mesh to guide point cloud editing. Compared to existing method, our framework are more efficient due to the neural point cloud representation and can be easily generalized to other editing tasks including relighting and scene composition.






% In a neural radiance representation, the spatial geometry and texture are directly encoded in a single MLP, thus shape manipulations are challenging. Our idea is to fully decouple the objects and lights, and encode the local geometry and material properties onto an explicit point cloud. Therefore, we can apply the classical physically based volume rendering instead of estimating the final color, while facilitating editings using the explicit shape. 



\ruofan{\textbf{Results \& Summary}: added later...}
% Make it strong.
% To the best of our knowledge, this is the first work that explicitly addresses the NeRF

To the best of our knowledge, this is the first work that applies an explicit neural point cloud representation of the NeRF, which enables a high-quality light-aware deformation of the geometry of the object, while full editability is provided to users. The user-performed deformation and learned illumination effects are able to be combined effectively to generate satisfying results with reasonable shadow effects on the deformed scene and not extensively losing the quality of the rendered images. Meanwhile, the training and rendering speed of our method are also sufficiently fast compared to the prior work. 

% maybe high-quali light-aware deformation is a good term to describe? yes
\ruofan{\textbf{Constributions}}






































% To answer the following questions:

% \textbf{What do we want to do?}
% Enable editing or deformation of NeRF models with one static scene as input. The rendered images after editing should remain photorealistic and correctly show the changes of lighting and shadow effect.

% \textbf{What are the challenges?}
% The NeRF-based implicit representation lacks \textcolor{red}{the} editability, since the coordinates that represents spatial geometry are encoded in the neural network. 
% The NeRF model implicitly encodes all the lighting effects into its implicit volume, even if we can make some deformations to the represented scene, these lighting effects cannot change accordingly.

% \textbf{How existing work address these problems?}
% Two fold:
% 1) To improve the editability on the shape/geometry:
% \begin{enumerate}
%     \item implicit nn model + explicit representation
%     \item GAN based generative approach.
%     \item learn from dynamic scenes.
% \end{enumerate}
% But still lacks finer-grained control.

% 2) To give the editability on the lighting effect:
%     combine concepts in photorealistic rendering to expliciting model/predict the lighting factors.
% This is an ill-posed problem. existing work show some promising results but still on low-resolution, coarse shapes.

% And there is no existing work that considers the both two.
    
% \textbf{What is our method?}
% Inspired by Point-NeRF, we use \textcolor{red}{a} point cloud based explicit representation plus implicit neural representation to render the target scene. Point cloud gives fine-grained manipulation over the learnt object.
% To decouple the lighting effect from the radiance field, we also capture the normal and light visibility from the environmental light map in order to perform a differentiable BRDF-based rendering process.

% \textbf{How novel our method is?}
% We introduce the normal prediction in the implicit-explicit hybrid NeRF model. Further integration with traditional rendering pipeline to ensure light-dependent and geometry-dependent rendering results. 

% \textbf{How about experiments?}
% \begin{enumerate}
%     \item Results of our improved pointNeRF, including SDF-based pruning for better point-surface alignment, predicted smooth normal map, etc.
%     \item Editing results:
%         \begin{enumerate}
%             \item manually editing points
%             \item physics-based simulation
%             \item object compositing.
%             \item relighting.
%         \end{enumerate}
% \end{enumerate}

% \textbf{Contribution}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> method_light_v0.tex <==
\section{Decomposing Lighting and Reflectance}\label{sec:lighting}
In this section, we describe how we decompose the reflectance and environment light from fully trained SDF-based PointNeRF models described in Sec. \ref{sec:sdf_pnerf}. There are three key components in our lighting estimation method. Firstly, we use an HDR light probe image encoded as a coordinate-based MLP to represent the environment light; Secondly, we employ the shadow mapping technique to approximate the surface light visibility; Lastly, we add 3 more MLP branches to estimate the surface BRDF property.


% After obtaining a trained SDF-based PointNeRF, the next step in our workflow is to decompose the environment light from the NeRF model for performing light-aware object deformation.
% Since NeRF encodes all the radiance information (including visibility, BRDF, environment light, etc.) into its neural volume, the shading color does not change when the object geometry is deformed. For example, the shadow in NeRF's rendering does not update when the deformation is applied to the object or the environment light changes (see Fig {\color{red} TODO}). 
% To make the shading color update in accordance with the object deformation, we have to make NeRF model compatible with the rendering methods used in the traditional computer graphics pipeline. 

% Mathematically, the outgoing radiance of a surface point $\mathbf{x}$ with normal $\hat{\mathbf{n}}$ from outgoing direction $\hat{\bm{\omega}}_o$ can be described by the classic rendering equation \citep{kajiya1986rendering}:
% \begin{equation}
%     L_o(\mathbf{x}, \hat{\bm{\omega}}_o) = \int_{\Omega}  L_i(\mathbf{x},  \hat{\bm{\omega}}_i) B(\mathbf{x}, \hat{\bm{\omega}}_i, \hat{\bm{\omega}}_o) (\hat{\mathbf{n}}\cdot \hat{\bm{\omega}}_i)  d \hat{\bm{\omega}}_i \label{eq:re}
% \end{equation}
% where $\hat{\bm{\omega}}_i$ denotes incoming light direction, $L_i(\mathbf{x},  \hat{\bm{\omega}}_i)$ is the incoming radiance of $\mathbf{x}$ from $\hat{\bm{\omega}}_i$, $B(\mathbf{x}, \hat{\bm{\omega}}_i, \hat{\bm{\omega}}_o)$ is the reflectance (BRDF) function that describes the portion of reflected radiance at direction $\hat{\bm{\omega}}_o$ from direction $\hat{\bm{\omega}}_i$, $\Omega$ denotes the hemisphere centered at $\hat{\mathbf{n}}$.
% {\color{red}TODO: add mode assumptions before further illustration, e.g., no emitting light, no indirect illumination, no semi-transparent, distant illumination...}
% We can directly obtain the normal direction $\hat{\mathbf{n}}$ from the NeRF model, and view direction $\hat{\mathbf{v}}$ in NeRF can be treated as the inverted outgoing direction (i.e., $\hat{\bm{\omega}}_o = -\hat{\mathbf{v}}$),  but the rest terms in the Eqn. \ref{eq:re} require extra modeling, which makes it a highly ill-posed problem. 

% Firstly, the incoming radiance term $L_i(\mathbf{x},  \hat{\bm{\omega}}_i)$ needs to consider the light directions $\hat{\bm{\omega}}_i$ over the whole hemisphere $\Omega$. Given a fixed light source outside of the object, not all the points $\mathbf{x}$ can receive the direct illumination of the light source due to the lighting occlusion caused by the object geometry. Therefore, we need to consider both global environment light $\bm{E}$ and point-level lighting visibility $\bm{V}$ to model the incoming radiance $L_i$. Since our goal includes hard shadow updates for the deformed object, the parameterization of $\bm{E}$ and $\bm{V}$ should be easy and straightforward for the geometry deformation. Inspired by NeRFactor \citep{nerfactor}, we choose the HDR light probe image  \citep{debevec1998rendering} to represent the environment light (Sec. \ref{sec:hrdi}). As for the surface visibility map, it is directly obtained from the geometry learned by our NeRF without training new models (Sec. \ref{sec:vis}).

% Secondly, the reflectance term $B(\mathbf{x}, \hat{\bm{\omega}}_i, \hat{\bm{\omega}}_o)$ is another challenging part in our rendering. The reflectance includes view-independent Lambertian reflection (diffuse) and view-dependent specular reflection. The Lambertian reflection has view-invariant BRDF which is fully controlled by the albedo $\mathbf{a}(\mathbf{x})$ of the corresponding surface point $\mathbf{x}$, while the non-Lambertian reflection has spatially-varying BRDF $f_r$ that depends on surface orientation/normal and surface material (e.g., roughness, IOR, etc.), which is hard to accurately estimate under such extremely constrained condition. Since our goal of learning reflectance is to achieve shading color update in accordance with objection deformation rather than relighting or material editing, 
% we simply map the specular color $\mathbf{c}_s$ learned from NeRF to a microfacet model \citep{walter2007microfacet} { \color{blue} or a single spherical Gaussian distribution} as a rough approximation of BRDF. The detailed modelings of parameters used in the reflectance are discussed in Sec. \ref{sec:ref}.

% {\color{red}TODO: maybe describe how we get the surface point here...}
% % We have to estimate the unknown illumination environment ($L_i$ term) as well as the reflectance property ($B$ term) from a collection of captured images of a static object under the same illumination environment.

% % $\hat{\bm{\omega}}_o = -\hat{\mathbf{v}}$ denotes outgoing direction, 
% % add equations.
% % how these components are combined together, then separately describe each one.

% In the following subsections, we give detailed descriptions of how we approximate the environment light, visibility map, and BRDF based on our NeRF model.

\subsection{Implicit Neural Environment Light\label{sec:hrdi}}
Similar to NeRFactor \citep{nerfactor}, a low-resolution HDR light probe image is used to represent the environment light. Every pixel on the light probe image can be treated as a distant light source on a sphere, thus the integral in the rendering equation (Eqn. \ref{eq:re}) can be discretized as the summation over a hemisphere of the light sources (pixels) on the light probe image. For practical reasons, our environment light is of $16 \times 32$ resolution in the latitude-longitude format, which can be treated as 512 point light source locations on a sphere centered around the object. As shown in NeRFactor, such a low-resolution light probe image is sufficient to capture the environment illumination with adequate high-frequency light components for synthesizing hard shadows.

Unlike NeRFactor directly optimizing 512 pixels $\mathbf{p}_i$ as learnable parameters, we instead use a simple coordinate-based MLP $E$ to implicitly represent the light probe. Given the $i$th light source's direction $\hat{\bm{\omega}}_i$ (normalized coordinate on a unit sphere), MLP $E$ takes $\hat{\bm{\omega}}_i$ as input (with positional encoding \citep{mildenhall2020nerf}) to predict the corresponding HDR pixel value $\mathbf{p}_i = E(\hat{\bm{\omega}}_i)$. Just like NeRF itself implicitly represents 5D radiance, such neural implicit representations for 2D light probes can better learn high-frequency signals while maintaining spatial smoothness \citep{tancik2020fourier, sitzmann2020implicit}.  

\subsection{Computing Visibility from Depth\label{sec:vis}}
% Unlike existing work that estimates point visibility with a visibility MLP \citep{nerv2021, nerfactor}, we directly use a visibility map computed based on the geometry learned from our SDF-based NeRF model. Though the MLP representation can improve the quality and reduce the noise of visibility maps, such an MLP representation is only applicable to the underlying fixed geometry, and is very hard to predict the updated visibility maps after geometry deformation, since the visibility map depends not only on the orientation of a local surface point but also on the occlusion of the global geometry that cannot be sensed by an MLP model implicitly encoding local spatial information. 
% Another benefit of using MLP representation is to reduce the cost of computing the visibility map for each surface point/pixel during rendering, since directly marching every one of 512 light sources to each surface point is a huge computation overhead.
% Therefore, we have to perform some pre-computation of the visibility map before rendering.

There are two potential ways to compute visibility maps. The first way is to directly compute visibility for each surface point by ray marching from 512 light source positions to the surface point \citep{bi2020neural, nerfactor}. The accumulated opacity from NeRF's volume rendering can be used as the visibility value for the corresponding light-surface point pair. The second way is to use shadow mapping, a common method in computer graphics \citep{williams1978casting, eisemann2013efficient}, to recover the per-point visibility maps from shadow maps of all light sources. The shadow maps are computed by comparing the depth difference between the depth map (z-buffer) from the view direction and the depth maps from the light sources after projecting to the same coordinate system. 
Compared to the first solution, the shadow mapping method could yield less accurate visibility maps due to projection and interpolation, but the latter solution has much less computation overhead (only need pre-compute one depth map for each light source). Considering that a low-resolution light probe image is used and object deformation requires frequent updates of visibility maps, we decide to use shadow mapping for computing visibility maps. Similar to other NeRF models, we use the expected termination of each camera ray from NeRF's ray marching to compute the depth map $\bm{D}$. Given the depth map $\bm{D}_c$ of the image captured by a camera with pose $\bm{T}_c$, and the depth maps $\bm{D}_{\bm{\omega}_i}$ of light sources with pose $\bm{T}_{\bm{\omega}_i}$, a pixel $(u, v)$ that represents a surface point $\mathbf{x}$ from the camera $\bm{T}_c$ has the shadow $\bm{S}(u, v, \hat{\bm{\omega}}_i)$ for the $i$th light source:
\begin{equation}
   \bm{S}(u, v, \hat{\bm{\omega}}_i) = \mathbf{1}\left\{\text{interp}(\bm{D}_{\bm{\omega}_i}^{\prime}, u,v) - \bm{D}_c(u,v) + b\right\}
\end{equation}
where $\mathbf{1}\{\cdot\}$ is a zero-one indicator function, $\bm{D}_{\bm{\omega}_i}^{\prime} = \bm{T}_{c}\bm{T}_{\bm{\omega}_i}^{-1}\bm{D}_{\bm{\omega}_i}$, representing the depth maps after projecting to $\bm{T}_c$'s coordinate system, $b$ is the shadow bias term, $\text{interp}(\cdot)$ represents a bi-linear interpolation function. The visibility map $\bm{V}$ is a collection of values from shadow maps of all light sources $\bm{V}(\mathbf{x}, \hat{\bm{\omega}}_i) =\bm{S}(u, v, \hat{\bm{\omega}}_i)$. With the help of the visibility map and light probe image, the  rendering integral (Eqn. \ref{eq:re}) can be approximated as 
\begin{align}
        L_o(\mathbf{x}, \hat{\bm{\omega}}_o) \approx \sum_{\hat{\bm{\omega}}_i}  L_i(\mathbf{x},  \hat{\bm{\omega}}_i) B(\mathbf{x}, \hat{\bm{\omega}}_i, \hat{\bm{\omega}}_o) (\hat{\mathbf{n}}\cdot \hat{\bm{\omega}}_i)  \Delta \hat{\bm{\omega}}_i \notag \\ 
        =\sum_{\hat{\bm{\omega}}_i} E(\hat{\bm{\omega}}_i) V(\mathbf{x},  \hat{\bm{\omega}}_i) B(\mathbf{x}, \hat{\bm{\omega}}_i, \hat{\bm{\omega}}_o) (\hat{\mathbf{n}}\cdot \hat{\bm{\omega}}_i)  \Delta \hat{\bm{\omega}}_i 
        \label{eq:re_sum}
\end{align}
where $\Delta \hat{\bm{\omega}}_i$ denotes the solid angle for the corresponding incoming light direction $\hat{\bm{\omega}}_i$ from the light probe image's hemisphere.

\subsection{Estimating BRDF from NeRF's Color Branches\label{sec:ref}}
Reflectance is the last important component we need to parameterize. Following the setup of microfacet BRDF models, the reflectance can be split into diffuse (Lambertian) and specular components. 
\begin{equation}
    B(\mathbf{x}, \hat{\bm{\omega}}_i, \hat{\bm{\omega}}_o) = \underbrace{\frac{\mathbf{a}(\mathbf{x})}{\pi}}_{\text{diffuse}} + \underbrace{\vphantom{\frac{\mathbf{a}(\mathbf{x})}{\pi}}f_r(\mathbf{x}, \hat{\bm{\omega}}_i, \hat{\bm{\omega}}_o)}_{\text{sepcular}}
\end{equation}
Recall that our Point-NeRF model also decomposes output radiance into diffuse color and specular color (Eqn. \ref{eq:d+s}), which is consistent with the BRDF decomposition. The diffuse and specular MLP branches ($R_d$ \& $R_s$) after the training have the knowledge about the modeling integrated color from the corresponding reflectances, which serve as strong priors for estimating the corresponding BRDF parameters. Next, we show how we estimate BRDF parameters from NeRF's color branches.

\noindent\textbf{Lambertian Reflectance}. View-independent diffuse reflectance is determined by the albedo $\mathbf{a}(\mathbf{x})$. Though albedo and diffuse color are completely different concepts, they have strong connections. Diffuse color $\mathbf{c}_d(\mathbf{x})$ is the integral result of Lambertian reflectance.
\begin{equation}
    \mathbf{c}_d(\mathbf{x}) 
    \approx \frac{\mathbf{a}(\mathbf{x})}{\pi} \sum_{\hat{\bm{\omega}}_i} E(\hat{\bm{\omega}}_i) V(\mathbf{x},  \hat{\bm{\omega}}_i) (\hat{\mathbf{n}}\cdot \hat{\bm{\omega}}_i)  \Delta \hat{\bm{\omega}}_i  
\end{equation}
For an ideal case where $\bm{E}=1, \bm{V}=1$ for all $\hat{\bm{\omega}}_i$, the diffuse color will be equal to the albedo $\mathbf{c}_d(\mathbf{x}) = \mathbf{a}(\mathbf{x})$, thus the diffuse color predicted by MLP $R_d$ can be a good initial estimation of the albedo. During the BRDF training step, MLP branch $R_d$ with its trained parameters is re-used to learn the albedo instead of the diffuse color. 
Note that accurate albedo estimation from one unknown illumination is an extremely difficult task, especially for an object with strong shadows, since the shadows can be ambiguously interpreted as the texture color (e.g., baked shadows). Therefore, we do not expect our model to be able to explain away the shadows completely, instead, we just want our simple albedo model can reduce the effect of the existing shadows from training images as much as possible when performing the object deformation. {\color{red} Maybe mention the NeRFactor's learning method.}

{\color{red}Maybe add point diffuse color regression...}

\noindent\textbf{Specular Reflectance.}
% Specular Reflectance is more difficult to estimate since it depends on more parameters to describe the reflection behavior of an object with varied materials. For simplicity, we want to use a simple and efficient BRDF model for rendering the specular color.
% Following the existing work \citep{bi2020neural, nerv2021}, we choose the microfacet BRDF \citep{walter2007microfacet} to parameterize the specular reflectance, so the specular BRDF $f_r$  at surface point $\mathbf{x}$ is parameterized by the roughness $\alpha$, the surface normal $\hat{\mathbf{n}}$, as well as material's normal incidence $F_0$. 
% Since microfacet BRDF is an analytical BRDF model, which means it can be differentiable, we can let neural models learn specular BRDF's parameters via gradient optimization.
% Next, we show how we model these additional parameters for microfacet BRDF.

% The roughness $\alpha$ is the first unknown parameter we need to estimate. The roughness is a scalar value used in microfacet's distribution functions (e.g., GGX distribution).  Considering the roughness values should have low variance over the entire surface of the same material, we simply attach a learnable roughness scalar to each neural point in the point cloud representation. Similar to the normal vector attached to the neural point, the roughness of a queried point is the inverse-distance interpolation of neighboring points' roughness, and the final roughness for a surface point also uses alpha-compositing weights $w_{\mathbf{x}}$ for the weighted sum.

% The material's normal incidence $F_0$ is used in the Fresnel term (Schlick's approximation) for simulating the way light interacts with a surface at different angles. 
% Depending on the type of the material (e.g., dielectric and conductor), $F_0$ can be approximated as a blend between default reflectance for dielectrics and base color for metals \citep{cook1982reflectance}. 
% % A common trick used in computer graphics is to make $F_0$ a blend between default reflectance for dielectrics and base color for metals \citep{mcauley2012practical} with a control parameter metalness. 
% As a rough estimation of specular BRDF, our model cannot precisely model those physics-related parameters. For simplicity, $F_0$ is directly modeled as a 3-D vector (similar to the albedo) for each surface point.
% $F = F_0 + (1-F_0)(1-\cos\theta)^5$, where $\theta$ is the angle between $\hat{\bm{\omega}}_o$ and half vector $\bm{h} = \hat{\bm{\omega}}_o + \hat{\bm{\omega}}_i$. 
Unlike roughness whose value changes have relatively less impact on the final rendered image, $F_0$ is more sensitive to the value changes. Due to this reason, we use an MLP branch to predict $F_0$ parameters.
Recall that we have an MLP branch $R_s$ specifically for the specular color during the NeRF training. $R_s$ is able to learn decent non-Lambertian view-dependent radiance for the target object. Utilizing the knowledge learned from $R_s$ should be beneficial for our specular BRDF estimation. Next, we build the connection between specular color $\mathbf{c}_s$ from $R_s$ and the microfacet rendering equation.

Analogous to diffuse color $\mathbf{c}_d(\mathbf{x})$, specular color $\mathbf{c}_s(\mathbf{x})$ can be treated is the integral result of the microfacet specular reflectance. Following the 
idea of \citep{karis2013real, boss2021neural}, $\mathbf{c}_s(\mathbf{x})$ can be approximated with split sum when $\bm{E} = 1$ and $\bm{V} = 1$
{
% \small
\begin{equation}
    \mathbf{c}_s(\mathbf{x}) \approx \sum_{\hat{\bm{\omega}}_i} \left(F_0  B_0(\hat{\bm{\omega}}_i, \hat{\bm{\omega}}_o) + B_1(\hat{\bm{\omega}}_i, \hat{\bm{\omega}}_o)\right)  (\hat{\mathbf{n}}\cdot \hat{\bm{\omega}}_i)  \Delta \hat{\bm{\omega}}_i 
    % + \sum_{\hat{\bm{\omega}}_i} B_1(\hat{\bm{\omega}}_i, \hat{\bm{\omega}}_o)  (\hat{\mathbf{n}}\cdot \hat{\bm{\omega}}_i)  \Delta \hat{\bm{\omega}}_i
\end{equation}
}
where $B_0$ and $B_1$ denote different combinations of the terms in the microfacet model.
Based on this approximation, $F_0$ can be represented as a function of $\mathbf{c}_s(\mathbf{x})$
\begin{equation}
    F_0(\mathbf{x}) \approx \frac{\mathbf{c}_s(\mathbf{x}) - \sum_{\hat{\bm{\omega}}_i} B_1(\hat{\bm{\omega}}_i, \hat{\bm{\omega}}_o)  (\hat{\mathbf{n}}\cdot \hat{\bm{\omega}}_i)  \Delta \hat{\bm{\omega}}_i}{\sum_{\hat{\bm{\omega}}_i} B_0(\hat{\bm{\omega}}_i, \hat{\bm{\omega}}_o) (\hat{\mathbf{n}}\cdot \hat{\bm{\omega}}_i)  \Delta \hat{\bm{\omega}}_i }
\end{equation}
We use this equation to get the $F_0(\mathbf{x})$'s initial estimation for the BRDF-based rendering, and MLP branch $R_s$ also gets optimized through this equation during the training.
Since $\mathbf{c}_s(\mathbf{x})$ is a view-dependent output of $R_s$ MLP branch, our approximated $F_0$ can be more or less affected by view direction $\hat{\bm{\omega}}_o$, even though $F_0$ should be a view-independent parameter by its physical definition. 
This is one of the compromises of our method for utilizing NeRF's view-dependent branch to estimate BRDF parameters. 
Also note that terms $B_0$ and $B_1$ also depend on view direction $\hat{\bm{\omega}}_o$. These terms altogether can make estimated $F_0(\mathbf{x})$ relative stable to the varying view directions.

{\color{red} This section should be aggressively compressed...}

\subsection{Training}
The training of light decomposition is based on the normally trained NeRF model from Sec. \ref{sec:train_s1}. 
% We first capture the depth maps $\bm{D}$ from the views of light sources on the light probe images. These depth maps are directly used for surface visibility computation, which also means we do not further update the NeRF's learned geometry thereafter.
Since this lighting-related training process involves a lot of parameter estimations, it is difficult to optimize the whole neural model directly. Not all the estimations need to be updated in this training. For example, the object geometry including depth information and normals is already well learned in NeRF's training and does not need further optimization, moreover, frequent updates on the geometry can cause a very high computation overhead for light depth maps and computed surface normals. 
Therefore, we freeze the geometry of the learned object and only optimize radiance related parameters. The object geometry is predicted by NeRF's density/SDF MLP branch and is mainly used in three places for our lighting-related training: 1) light depth maps, 2) point normals, 3) alpha-compositing weights.
As the geometry is frozen in this training process, we can use pre-computed light depth maps for computing visibility throughout the training, and also use point-attached normals (Sec. \ref{sec:point_normal}) for normal-related operations. 
However, the challenging part is how to remain the alpha-compositing weights $w_{\mathbf{x}}$ unchanged. Because NeRF's density MLP branch outputs not only density values but also neural features fed to radiance branches, fixing the whole density branch can significantly limit the optimization space for radiance parameters (features attached to neural points cannot get optimized either). 
% especially for a hybrid NeRF model with a large portion of neural parameters from the discrete representation.
To address this issue, we propose a two-step training process. In the first step, we completely freeze the density branch and only optimize two radiance branches ($R_d$ \& $R_a$) to predict the corresponding BRDF parameters.
In the second step, we jointly optimize all the neural parameters in our model. To avoid the geometry updates in this joint training, we additionally run a frozen copy of density branch $T^*$ to output unchanged weights $w_{\mathbf{x}}^{*}$. These frozen weights $w_{\mathbf{x}}^{*}$ can also form a distillation/regularization loss $\mathcal{L}_g(w_{\mathbf{x}}^{*}, w_{\mathbf{x}})$ to constrain the geometry changes while updating neural features for BRDF predictions.
A simple L1 color loss $\mathcal{L}_{color}$ is used in the light training (the second step also includes geometry regularization $\mathcal{L}_g$).

The neural implicit light model is a relatively independent MLP model, it gets gradient optimization only from our differentiable rendering equation (Eqn. \ref{eq:re_sum}). Since it models HDR images, we adopt the exponential activation \citep{mildenhall2022nerf} to convert MLP output to the final HDRI. Besides, we initialize this MLP model so that the initial light probe representation is close to the all-one light probe $\bm{E} = 1$, which enables a smooth transition of radiance branches from predicting color to predicting BRDF parameters.



==> related_work_v0.tex <==
\section{Related Work}

\textbf{Scene representations and neural rendering.} 
% Synthesizing images from novel unobserved viewpoints given a set of captured scene images is a long-standing task in computer vision and graphics. 
3D scene representation is one of the core research topics in computer vision and graphics. To model a 3D scene for synthesis, methods with explicit or implicit representations have been proposed. 
Explicit methods describe scenes with a set of geometric primitives such as triangles \citep{debevec1996modeling, wood2000surface, waechter2014let}, voxels \citep{sitzmann2019deepvoxels, lombardi2019neural, rematas2020neural}, and points \citep{aliev2020neural, dai2020neural}. Implicit methods on the other hand use implicit functions such as occupancy and signed distance functions \citep{chen2019learning, mescheder2019occupancy, park2019deepsdf} to describe the scene geometry. 
% The synthesized images are the rendered results of different scene representations via rendering methods such as rasterization and raytracing.
%Though the direct rendering with explicit representations is still the most widely used rendering method in games and videos,
% Unlike classical rendering approaches,
Neural rendering is a class of reconstruction and rendering approaches that use deep networks to learn complex mappings from captured images to novel images \citep{tewari2020state}.
The recent progress in neural rendering has shown promising results in various tasks such as texture mapping \citep{thies2019deferred}, surface reconstruction \citep{yariv2020multiview}, image generation \citep{chan2022efficient}, etc. 
Neural radiance field (NeRF) \citep{mildenhall2020nerf} is one representative work that shows how the current state-of-the-art methods \citep{barron2021mip, barron2022mip, verbin2021ref} combine volume rendering and neural network based implicit representation for photo-realistic novel view synthesis. Follow-up methods that combine surface SDF estimation and neural volume rendering \citep{yariv2021volume, wang2021neus} further improve the quality of surface reconstruction that the original NeRF performs not well.
% In addition to using one global MLP to parameterize the whole scene, 
In order to make NeRF's training and rendering more efficient, hybrid neural representations that combine implicit MLP and other discrete spatial representations such as voxel grids \citep{liu2020neural, sun2022direct, fridovich2022plenoxels}, point cloud \citep{ost2022neural, xu2022point} and hash table \citep{mueller2022instant} have been proposed and achieved significant speed boost.
However, these hybrid representations usually lack the ability to well maintain the surface geometry (e.g., surface normal) because of using relatively coarse-grained discrete spatial representation and adoption of the original NeRF's volume rendering equation. Our point-based hybrid neural representation with SDF-based volume rendering in this case can provide better surface reconstruction while maintaining relatively high computing efficiency.
% 

% The mathematical description of scene representation has been a hot research topic in the academic community. Many scene representations exist in computer graphics, such as point clouds and meshes. These explicit representations are widely used in mature industrial streams since they have strong editing properties and can be easily applied in traditional rendering pipelines, which provide a great deal of convenience for the customer. 
% These representations require much manual design to achieve high fidelity. By contrast, neural scene representations can perform high fidelity with poor interoperability and edibility. 
% Such scene representations leverage calibrated images, videos, point clouds, or a combination of the above to reconstruct the physics distribution of the scene.
% Generally, neural scene representations implicitly represent scene components as outputs of neural networks. 
% Existing approaches propose a differentiable mapping equation (usually a neural network) to map discrete geometric primitives to n-dimensional feature space and then render the accumulated spatial properties into pixel space utilizing volume rendering.
% \citep{mildenhall2020nerf},~\citep{mipnerf},~\citep{mip360},~\citep{NSVF},~\citep{NGP}~utilize neural volumetric representations to represent the scenes. In this case, the space consists of a continuous density field and its corresponding color field. 
% \citep{deepsdf},~\citep{IDR},~\citep{volsdf},~\citep{neuS},~\citep{manhattansdf},~\citep{monosdf},~\citep{neuris}~use a network's zero-level set to define the surface in continuous space. 


\textbf{Geometry editing and deformation.}
3D geometry modeling and editing is a popular topic in computer graphics. Prior works mainly focus on the editing of explicit scene representations, such as object movement \citep{karsch2011rendering, kholgade20143d} and deformation \citep{sorkine2007rigid, jacobson2012fast, yifan2020neural}. However, those editing methods cannot be directly applied to 3D neural implicit representations such as NeRF. The use of deep neural networks as implicit functions limits the explicit control such as movement and deformation over the represented scene geometry. With the emergence of NeRF, methods that specifically tackle NeRF's geometry editability or deformation have been proposed. 
For geometry editability, scene composition is one type of editing that has been discussed by several works \citep{liu2020neural, guo2020object, yang2021learning, tang2022compressible}. Although these editing methods allow users to add or move objects in the scene, the shape of each individual object in the scene can be changed.
% There are works attempting to learn deformable NeRF representations from dynamic scenes by warping canonical coordinate space \citep{pumarola2021d, park2021nerfies} or mapping representation to higher-dimensional space \citep{park2021hypernerf}. Since these works learn the deformation from the input data, thus they do not support user-defined explicit geometry control. 
Recent works also explore ways to perform user-defined geometry deformation for NeRF representations. \cite{liu2021editing} takes an optimization approach to realize the shape editing on the simple objects belonging to certain categories \citep{chang2015shapenet}. Closest to our approach are \cite{Yuan22NeRFEditing, neumesh}, where they achieve more flexible object deformations by using mesh-guided geometry deformation. Different from their methods, our method uses point cloud as explicit representations, which means users can use not only mesh (reconstructed from points or using marching cube method) but also point cloud for various geometry editing such as non-rigid body deformation, fine-grained rigid body transformation, object inserting and removing, etc. Beyond the scope of geometry editing, there are few existing works that address the illumination or lighting changes after the geometry editing for neural implicit representations. 
\cite{guo2020object} model the light scattering function for composing scenes under different lighting conditions, but this method assumes the light source is known before training and cannot perform per-object geometry editing.
In contrast, our method further provides a solution for general geometry editing with lighting-aware rendering, by learning the decomposed lighting from the NeRF representation.

\textbf{Lighting estimation.}
Lighting estimation is a long-existing problem that aims to estimate surface reflectance properties and lighting conditions from captured or rendered images. This problem is also known as inverse rendering \citep{marschner1998inverse, ramamoorthi2001signal}. The surface reflectance property can be mathematically described by a bidirectional reflectance distribution function (BRDF). The precise BRDF estimation often relies on highly restricted laboratory conditions with known object geometry or controllable lighting \citep{lensch2001image, matusik2003data, lawrence2004efficient}. Recent works also leverage machine learning methods to alleviate these constraints for casual captures \citep{aittala2016reflectance, deschaintre2018single, gao2019deep}. However, most of these works still require known illumination for BRDF estimation. 
Environment light estimation also relies on the modeling of the interaction between light sources and surfaces. This line of work requires additional 3D geometry prior for high-fidelity environment estimation \citep{richter2016instant, legendre2019deeplight, park2020seeing}. 
Recent works that focus on reflectance in 3D neural implicit representations also pay more attention to scene lighting and material reflectance that are implicitly encoded in neural parameters. \cite{bi2020neural, nerv2021} attempt to learn the material reflectance properties with NeRF, but both methods require the known lighting conditions.
Our method also aims to learn the decomposition of scene lighting and material in NeRF, but simply with captured images under one unknown lighting condition. 
\cite{boss2021nerd, boss2021neural, zhang2021physg} share the same problem setup as our model, 
% decompose lighting and reflectance under unknown lighting conditions, 
but their lighting approximation methods (e.g., spherical Gaussian, pre-integrated maps) do not consider self-occlusions, thus cannot render shadowing effects caused by occlusion.
\cite{nerv2021, nerfactor} have explicit light visibility estimation in their model, enabling them to render relightable shadowing effects. However, the rendering results of these methods are over-smoothed and lack high-frequency details.
On the other hand, relighting is the main application for these NeRF extensions, and none of these aforementioned works can be applied to address the illumination changes caused by geometry editing in NeRF. 
Our method uses the shadow mapping technique to approximate the surface light visibility, which enables our model to show updated lighting and shadowing effects after editing the geometry of a NeRF scene. 
We also propose a new approach that represents HDR environment light probes as coordinate-based MLPs to effectively learn continuous, high-fidelity lighting conditions.
%is another challenging problem in inverse rendering. Since environment lighting is only observable through the interaction between light and surface, lighting estimation also relies on the surface BRDF properties. Those works that make lighting estimation also jointly model the surface BRDF. 





% The surface definition can represent objects with unknown topology or changing topology in a dynamic scenario. 
% Explicitly defining the surface can effectively constrain the spatial property distribution while enabling regularization terms on the gradients.
% ~\citep{NBPG},~\citep{ADOP},~\citep{Pulsar},~\citep{xu2022point}~use pointcloud with neural features as the representation of the scene. The point cloud is a set of elements of the Euclidean space, so the neural point cloud enables the representation of continuous scenes by interpolation in surface approximation or volume approximation. % maybe more about pointnerf?


% points and meshes has high edibility but has difficulty in achieving high fidelity, neural implicit functions (SDF \citep{Park_2019_CVPR}, NeRF \citep{mildenhall2020nerf}, NSVF \citep{liu2020neural}) high fidelity from RGB images, but poor interoperability and edibility.  


% \textbf{Mutli-view reconstruction / inverse graphics} 
% The process of taking photos converts 3D scenes to 2D images. Part of the scene information is inevitably lost in this procedure. In contrast, reconstructing the scene representation from observations is called inverse rendering or inverse graphics. The Multi-View Stereo (MVS) method attempts to match features and predict depth from images across views. Recently, \citep{yao2018mvsnet},~\citep{DeepMVS},~\citep{PatchmatchNet},~\citep{P-MVSNet},~\citep{Recurrent mvsnet} apply an end-to-end framework to reconstruct learning-based neural point clouds from multi-view input based on the plane-sweeping strategy. The neural point cloud generated from DeepMVS-like methods contains not only location details but also implies additional scene information. Through interpolation or growing, the neural point cloud can approximately describe continuous scenes while maintaining high interactivity and editable capabilities.
% depth based scanning (active scanning), deep learning based neural point clouds (MVS) \citep{DeepMVS}. 
% ~\citep{xu2022point},~\citep{ibrnet},~\citep{MVSnerf},~\citep{geonerf},~\citep{ProbNVS} try to combine neural implicit functions with MVS methods to achieve a more realistic and accurate scene representation.

% There are some method combining the MVS method and neural implicit functions (ibrnet, MVS nerf, geonerf).


% \textbf{Relighting and interactive shape editing} 
% % hmmmmm
% \textcolor{red}{relighting and shape?}

% maybe some hint ?

% Editing Conditional Radiance Fields, GIRAFFE \citep{Niemeyer2020GIRAFFE}, Nerfie \citep{park2021nerfies}, NeRV \citep{nerv2021}, Nerfactor \citep{nerfactor}, 
% Learning Object-Compositional Neural Radiance Field

% for Editable Scene Rendering \citep{yang2021objectnerf}.  
% domain-specific, limited edibility, intensive computations at inference time. 

% compared to \textbf{NeRF-Editing: Geometry Editing of Neural Radiance Fields}


==> tables/blendedMVS_perscene.tex <==
\begin{table}[]
\centering
\small
\caption{Per-scene Quantitative Results on BlendedMVS}
\begin{tabular}{c|cccc}
\hline
&\multicolumn{4}{c}{Blended MVS}                                         \\
                               & Jade  & Fountain & Character & Statues \\ \hline
\multicolumn{5}{c}{\textbf{PSNR $\uparrow$}}                                       \\ \hline
\multicolumn{1}{c|}{NSVF}      & 26.96 & 27.73    & 27.95     & 24.97   \\
\multicolumn{1}{c|}{VolSDF}    & 25.20 & 24.05    & 25.59     & 24.26   \\
\multicolumn{1}{c|}{PointNeRF} & 26.14 & 25.68    & 29.06     & 25.97   \\
\multicolumn{1}{c|}{Ours}      & 25.70 & 27.25    & 27.80     & 25.50   \\
\multicolumn{1}{c|}{Ours-BRDF} & 25.70 & 26.29    & 25.42     & 23.95   \\ \hline
\multicolumn{5}{c}{\textbf{SSIM $\uparrow$}}                                       \\ \hline
\multicolumn{1}{c|}{NSVF}      & 0.901 & 0.913    & 0.921     & 0.858   \\
\multicolumn{1}{c|}{VolSDF}    & 0.919 & 0.908    & 0.939     & 0.895   \\
\multicolumn{1}{c|}{PointNeRF} & 0.931 & 0.935    & 0.970     & 0.930   \\
\multicolumn{1}{c|}{Ours}      & 0.933 & 0.957    & 0.968     & 0.933   \\
\multicolumn{1}{c|}{Ours-BRDF} & 0.919 & 0.950    & 0.950     & 0.910   \\ \hline
\multicolumn{5}{c}{\textbf{LPIPS $\downarrow$}}                                      \\ \hline
\multicolumn{1}{c|}{NSVF}      & 0.094 & 0.113    & 0.074     & 0.171   \\
\multicolumn{1}{c|}{VolSDF}    & 0.128 & 0.177    & 0.091     & 0.196   \\
\multicolumn{1}{c|}{PointNeRF} & 0.091 & 0.104    & 0.033     & 0.082   \\
\multicolumn{1}{c|}{Ours}      & 0.083 & 0.061    & 0.039     & 0.087   \\
\multicolumn{1}{c|}{Ours-BRDF} & 0.101 & 0.068    & 0.055     & 0.115   \\ \hline
% \multicolumn{5}{c}{\textbf{LPIPS\textsubscript{VGG} $\downarrow$}}                                   \\ \hline
% \multicolumn{1}{c|}{VolSDF}    & 0.163 & 0.186    & 0.095     & 0.196   \\
% \multicolumn{1}{c|}{PointNeRF} & 0.133 & 0.142    & 0.053     & 0.119   \\
% \multicolumn{1}{c|}{Ours}      & 0.114 & 0.088    & 0.052     & 0.113   \\
% \multicolumn{1}{c|}{Ours-BRDF} & 0.143 & 0.099    & 0.073     & 0.142   \\ \hline
\multicolumn{5}{c}{\textbf{MAE\si{\degree} $\downarrow$}}                                                                                                             \\ \hline
\multicolumn{1}{c|}{VolSDF}    & 32.17 & 24.87 & 28.74 & 18.03 \\
\multicolumn{1}{c|}{PointNeRF} & 48.62 & 43.15 & 58.30 & 54.61 \\
\multicolumn{1}{c|}{Ours-Grad} & 50.60 & 50.07 & 50.43 & 38.89 \\
\multicolumn{1}{c|}{Ours-Pred} & 42.39 & 34.42 & 33.96 & 27.42 \\ \hline
\end{tabular}
\label{tab:perscene_bmvs}
\end{table}






